Adaptive Draft-Verification for Efficient Large Language Model Decoding

Large language model (LLM) decoding involves generating a sequence of tokens based on a given context, where each token is predicted one at a time using the model's learned probabilities. The typical autoregressive decoding method requires a separate forward pass through the model for each token generated, which is computationally inefficient and poses challenges for deploying LLMs in latency-sensitive scenarios. The main limitations of current decoding methods stem from their inefficiencies and resource demands. Existing approaches either necessitate fine-tuning smaller models, which is resource-intensive, or rely on fixed retrieval schemes to construct drafts for the next tokens, which lack adaptability and fail to generalize across different models and contexts. To address these issues, we introduce a novel methodology called ADED, which accelerates LLM decoding without requiring fine-tuning. Our approach involves an adaptive draft-verification process that evolves over time to improve efficiency. We utilize a tri-gram matrix-based LLM representation to dynamically approximate the output distribution of the LLM, allowing the model to adjust to changing token probabilities during the decoding process. Additionally, we implement a draft construction mechanism that effectively balances exploration and exploitation, ensuring that the drafts generated are both diverse and close to the true output distribution of the LLM. The importance of this design lies in its ability to optimize the draft distribution adaptively, leading to faster and more accurate decoding. Through extensive experiments on various benchmark datasets and LLM architectures, we demonstrate that ADED significantly accelerates the decoding process while maintaining high accuracy, making it suitable for deployment in a wide range of practical applications.

==> sections/7-checklist.tex <==
\newpage
\section*{Reproducibility Checklist}

\textbf{This paper:}
\begin{itemize}
    \item Includes a conceptual outline and/or pseudocode description of AI methods introduced \textbf{[yes]}
    \item Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results \textbf{[yes]}
    \item Provides well marked pedagogical references for less-familiar readers to gain background necessary to replicate the paper \textbf{[yes]}
\end{itemize}

\textbf{Does this paper make theoretical contributions? \textbf{[no]}}

% If yes, please complete the list below.
% \begin{itemize}
%     \item All assumptions and restrictions are stated clearly and formally. (yes/partial/no)
%     \item All novel claims are stated formally (e.g., in theorem statements). (yes/partial/no)
%     \item Proofs of all novel claims are included. (yes/partial/no)
%     \item Proof sketches or intuitions are given for complex and/or novel results. (yes/partial/no)
%     \item Appropriate citations to theoretical tools used are given. (yes/partial/no)
%     \item All theoretical claims are demonstrated empirically to hold. (yes/partial/no/NA)
%     \item All experimental code used to eliminate or disprove claims is included. (yes/no/NA)
%     \item Does this paper rely on one or more datasets? (yes/no)
% \end{itemize}

\textbf{Does this paper rely on one or more datasets? \textbf{[yes]}}

\begin{itemize}
    \item A motivation is given for why the experiments are conducted on the selected datasets. \textbf{[yes]}
    \item All novel datasets introduced in this paper are included in a data appendix. \textbf{[NA]}
    \item All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. \textbf{[NA]}
    \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations. \textbf{[yes]}
    \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available. \textbf{[yes]}
    \item All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing. \textbf{[NA]}
\end{itemize}

\textbf{Does this paper include computational experiments? \textbf{[yes]}}
\begin{itemize}
    \item Any code required for pre-processing data is included in the appendix. \textbf{[yes]}
    \item All source code required for conducting and analyzing the experiments is included in a code appendix. \textbf{[yes]}
    \item All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. \textbf{[yes]}
    \item All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from. \textbf{[yes]}
    \item If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. \textbf{[NA]}
    \item This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks. \textbf{[partial]}
    \item This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics. \textbf{[yes]}
    \item This paper states the number of algorithm runs used to compute each reported result. \textbf{[yes]}
    \item Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. \textbf{[yes]}
    \item The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank). \textbf{[no]}
    \item This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments. \textbf{[yes]}
    \item This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting. \textbf{[yes]}
\end{itemize}
